Lattice QCD Calculation of Electroweak Box Contributions to Superallowed Nuclear and Neutron Beta Decays

We present the first lattice QCD calculation of the universal axial $\gamma W$-box contribution $\square_{\gamma W}^{VA}$ to both superallowed nuclear and neutron beta decays. This contribution emerges as a significant component within the theoretical uncertainties surrounding the extraction of $|V_{ud}|$ from superallowed decays. Our calculation is conducted using two domain wall fermion ensembles at the physical pion mass. To construct the nucleon 4-point correlation functions, we employ the random sparsening field technique. Furthermore, we incorporate long-distance contributions to the hadronic function using the infinite-volume reconstruction method. Upon performing the continuum extrapolation, we arrive at $\square_{\gamma W}^{VA}=3.65(8)_{\mathrm{lat}}(1)_{\mathrm{PT}}\times10^{-3}$. Consequently, this yields a slightly higher value of $|V_{ud}|=0.97386(11)_{\mathrm{exp.}}(9)_{\mathrm{RC}}(27)_{\mathrm{NS}}$, reducing the previous $2.1\sigma$ tension with the CKM unitarity to $1.8\sigma$. Additionally, we calculate the vector $\gamma W$-box contribution to the axial charge $g_A$, denoted as $\square_{\gamma W}^{VV}$, and explore its potential implications.

==> Makefile <==
MAIN     = paper
FIGDIR   = 
DEPS     = Makefile $(wildcard *.sty)

$(MAIN).pdf: $(MAIN).tex figures $(DEPS) 
	latexmk -pdf $(MAIN).tex
	
%.pdf: $(DEPS)
	make -C $(FIGDIR) $@

.PHONY: figures dist arxiv template clean veryclean

#figures: $(DEPS)
#	make -C $(FIGDIR) all
	
dist: veryclean
	ARNAME=$(MAIN)_`date +%y%m%d`;\
	ln -s . $${ARNAME};\
	tar --exclude="$${ARNAME}/$${ARNAME}*" --exclude='.DS_Store'\
		--exclude="$(MAIN)*tar.bz2" -chjf $${ARNAME}.tar.bz2 $${ARNAME};\
	rm -f $${ARNAME}

arxiv: $(MAIN).pdf
	ARNAME=$(MAIN)_arXiv_`date +%y%m%d`;\
	tar --exclude="$(MAIN).pdf" -cjvf $${ARNAME}.tar.bz2\
		`find -name '*.tex' -o -name '*.bbl' -o -name '*.pdf' -o -name '*.sty'\
			  -o -name '*.cls' | grep -v '/src/'`

template:
	[ ! -e $(MAIN).tex ] && cp .template $(MAIN).tex
	
clean:
	latexmk -C
	rm -f $(MAIN).synctex.gz
	make -C $(FIGDIR) clean

veryclean: clean
	rm -f $(MAIN).pdf $(MAIN).bbl $(MAIN).nav $(MAIN).snm 
	make -C $(FIGDIR) veryclean

